Greedy PIG: Adaptive Integrated Gradients

Deep learning has become the standard approach for most machine learning tasks. While its impact is undeniable, interpreting the predictions of deep learning models from a human perspective remains a challenge. In contrast to model training, model interpretability is harder to quantify and pose as an explicit optimization problem. Inspired by the AUC softmax information curve (AUC SIC) metric for evaluating feature attribution methods, we propose a unified discrete optimization framework for feature attribution and feature selection based on subset selection. This leads to a natural adaptive generalization of the path integrated gradients (PIG) method for feature attribution, which we call Greedy PIG. We demonstrate the success of Greedy PIG on a wide variety of tasks, including image feature attribution, graph compression/explanation, and post-hoc feature selection on tabular data. Our results show that introducing adaptivity is a powerful and versatile method for making attribution methods more powerful.

==> notebook.tex <==
\section{Notebook}
\subsection{Contributions}
Contribution 1: Formulate feature importance as a subset selection problem. This formulation also generalizes feature importance with general loss functions and feature selection.
Contribution 2: Improve the above subset selection metric (e.g. AUC softmax information curve in previous work) by directly solving the subset selection problem (with Greedy PIG), instead of using PIG.
Contribution 3: Propose new loss functions that produce more interpretable results. For example minimize cross entropy to the target distribution, instead of maximizing softmax of target class.
Contribution 4 (Maybe): Explore the tradeoff between adaptivity (number of rounds) and number of gradient evaluations per round. Contribution 5: Challenge the notion that PIG fails because of "noise" in the data, instead proposing that it is because of feature correlations. We can show some theoretical evidence for this using PIG on linear regression. Basically a) if we have two features that are highly correlated, PIG scores will be unbounded (but cancel out), so high correlation breaks PIG and b) we have two uncorrelated features and can replicate both of them many times such that their PIG scores' order is flipped. This also breaks PIG but not Greedy PIG. Probably it also breaks the de-noising approaches from previous work.


Experiment 0: Show that PIG fails with linear regression when replicating features (while Greedy PIG does not fail). Also show similar behavior by replicating edges/nodes in graphs?
Experiment 1: Compare AUC softmax information curve on imagenet with the mobilenetV2 (?) pretrained model. This is a per-instance metric, which we can aggregate over the whole dataset, as done in https://arxiv.org/abs/2106.09788.
Experiment 2: Apply for feature selection on criteo small and compare with other methods. This can be done by running Greedy PIG / PIG on the expected cross entropy loss over the whole training dataset. (In practice we just pull batches and update the average gradient, then at fixed intervals make a selection).
Experiment 3: Apply to graph learning problems (e.g. ogbn-arxiv?) to select most important edges,  @Sami Abu-el-haija knows more about this.
Experiment 4 (Maybe): Apply on youtube8m video dataset to find most important video frames.


\subsection{Related work}
\begin{itemize}
    \item \citet{kapishnikov2021guided}: Adaptive path-building algorithm that moves in the direction of noise?
    \item \citet{agarwal2022openxai}
    \item \citet{kapishnikov2019xrai}
\end{itemize}

\subsection{Math}

Consider PIG, in which scores are defined by
$\aa = -\int_{t=0}^1\nabla g(t\onev) dt$ for some function $g:[0,1]^n\rightarrow\mathbb{R}$ to be minimized.
PIG scores have the following property:
\begin{lemma}
Suppose there exists a feature cut $S\subset [n]$ such that the 
features in $S$ are not correlated to the features in 
$\bar{S} = [n]\backslash S$.
Then, 
$\sum\limits_{i\in S} a_i = g(\zerov) - g(\onev_S)$ and
$\sum\limits_{i\in \bar{S}} a_i = g(\zerov) - g(\onev_{\bar{S}})$
\end{lemma}
\begin{proof}
Let $\HH(\ww)$ be the Hessian of $g$ at $\ww$, for any $\ww$. 
The non-correlation
property implies that $(\HH(\ww))_{S\bar{S}} = \OO$.
Then, by Taylor's theorem we have
\[ \nabla g(\ww) = \nabla g(\ww_S) + \oHH \ww_{\bar{S}} \]
where $\oHH$ is an average Hessian on the path from $\ww$ to $\ww_S$.
However, by the non-correlation property this implies that
\[ \nabla_S g(\ww) = \nabla_S g(\ww_S) \]
As a result, we have that
\begin{align*}
\langle \onev, \aa_S \rangle
& = \langle \onev, -\int_{t=0}^1 \nabla_S g(t\onev) dt\rangle \\
& = \langle \onev, -\int_{t=0}^1 \nabla_S g(t\onev_S) dt\rangle \\
& = g(\zerov) - g(\onev_S)\,.
\end{align*}
\end{proof}



Suppose that the columns of $\XX$ and $\yy$ 
are scaled to unit $\ell_2$ norm.
We note that the marginal contribution of the $i$-th feature is
$\frac{1}{2}\left\langle \XX_i, \yy\right\rangle^2$.

Case 1: Suppose that the features are uncorrelated, i.e. 
$\langle \XX_i, \XX_j\rangle = 0$ for all $i\neq j$. Then, note that $a_i = -\nabla_i g(\zerov) = 
-(\vTheta\XX^\top(\XX\ww\vtheta - \yy))_i |_{\ww=\zerov}
= \theta_i \langle \XX_i, \yy\rangle$.
Now, as $\vtheta$ is the full linear regression solution, we have
$\vtheta = (\XX^\top \XX)^+ \XX^\top \yy$, and, since the features are
uncorrelated and scaled, $\XX^\top \XX = \II$, so $\vtheta = \XX^\top \yy$.
We conclude that $a_i = \langle \XX_i, \yy\rangle^2$, which is twice
the marginal contribution.

Case 2: Suppose that each feature is only correlated with $O(1)$ other
features. 

\begin{lemma}[Effects of redundancy]
Consider a function $g:[0,1]^n\rightarrow \mathbb{R}$. Given some
integers $k_1,\dots,k_n \geq 1$ we define a new function which corresponds
to replacing the $i$-th coordinate by $k_i$ identical copies, for all $i$.
Specifically, we define 
$h:[0,1]^{\sum k_i}\rightarrow \mathbb{R}$ as
\begin{align*}
& h(x_{11}, \dots, x_{1k_1}, x_{21}, \dots, x_{2k_2},\dots, x_{n1}, \dots, x_{nk_n})\\
& =
g(x_{11}+ \dots+ x_{1k_1}, x_{21}+ \dots+ x_{2k_2},\dots, x_{n1}+ \dots+ x_{nk_n})
\end{align*}. 

Let $s_i(g)$ be the PIG attributions of $g(\onev)$ with baseline $\zerov$
and $s_{ij}(h)$ the PIG attributions of
$h(\vv:=(1/k_1,\dots, 1/k_1, 1/k_2, \dots, 1/k_2,\dots))$ with baseline $\zerov$.
Then, $s_{ij}(h) = \frac{1}{k_i} s_i(g)$ for all $i, j$.
\end{lemma}
\begin{proof}
Note that $\nabla_{ij} h(\yy) = \nabla_i g(\xx)$ for any $\xx, i, j$. 
Therefore,
\[ s_{ij}(h)
= \int_{t=0}^1\nabla_{ij} h(t\vv)dt \cdot v_{ij}
= \int_{t=0}^1\nabla_{i} g(t\onev)dt \cdot \frac{1}{k_i}
= \frac{1}{k_i} s_i(g)
\]
\end{proof}
